Acquire and then Adapt: Squeezing out Text-to-Image Model for Image Restoration

Recently, pre-trained text-to-image (T2I) models have been extensively adopted for real-world image restoration because of their powerful generative prior. However, controlling these large models for image restoration usually requires a large number of high-quality images and immense computational resources for training, which is costly and not privacy-friendly. In this paper, we find that the well-trained large T2I model (i.e., Flux) is able to produce a variety of high-quality images aligned with real-world distributions, offering an unlimited supply of training samples to mitigate the above issue. Specifically, we proposed a training data construction pipeline for image restoration, namely FluxGen, which includes unconditional image generation, image selection, and degraded image simulation. A novel light-weighted adapter (FluxIR) with squeeze-and-excitation layers is also carefully designed to control the large Diffusion Transformer (DiT)-based T2I model so that reasonable details can be restored. Experiments demonstrate that our proposed method enables the Flux model to adapt effectively to real-world image restoration tasks, achieving superior scores and visual quality on both synthetic and real-world degradation datasets - at only about 8.5\% of the training cost compared to current approaches.

==> table/campare_ablation_T2I_IQA.tex <==
\begin{table}[h]\color{blue}
    \captionsetup{font=small}
    % \small
    \footnotesize
    \centering
    \renewcommand\arraystretch{0.8}
    \setlength\tabcolsep{2pt}
    \caption{Comparisons with existing T2I generation methods.}
    \vspace{-6pt}
    \begin{tabular}{c|cccccc}
        \toprule
        Metric & PixArt-$\Sigma$ & Sana & SDXL & Playground & Flux.1-dev & Ours \\
        \midrule
        CLIPIQA $\uparrow$ & 0.4981 & 0.5135 & 0.5821 & 0.5822 & 0.6763 & \textbf{0.7295} \\
        MUSIQ $\uparrow$ & 64.93 & 66.75 & 70.49 & 70.35 & 75.02 & \textbf{75.37} \\
        MANIQA $\uparrow$ & 0.5519 & 0.5944 & 0.5831 & 0.6666 & 0.6590 & \textbf{0.6962} \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation_T2I_IQA}
\end{table}
